Exploring and Evaluating Real-world CXL: Use Cases and System Adoption

Compute eXpress Link (CXL) is emerging as a promising memory interface technology. However, its performance characteristics remain largely unclear due to the limited availability of production hardware. Key questions include: What are the use cases for the CXL memory? What are the impacts of the CXL memory on application performance? How to use the CXL memory in combination with existing memory components? In this work, we study the performance of three genuine CXL memory-expansion cards from different vendors. We characterize the basic performance of the CXL memory, study how HPC applications and large language models (LLM) can benefit from the CXL memory, and study the interplay between memory tiering and page interleaving. We also propose a novel data object-level interleaving policy to match the interleaving policy with memory access patterns. Our findings reveal the challenges and opportunities of using the CXL memory.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 2.06.  Added eISSN for a number of journals.
               ACM no longer collects or prints authors'
	       postal addresses

Version 2.05   Changed title for TELO.

Version 2.04   Compatibility with the new latex-dev format
               eSSN is always printed, even if pSSN is present
	       Wording change in copyright statement

Version 2.03   Cleaned generation of samples.
	       New options for printing conference proceedings
	       in ACM journals

Version 2.02   Documentation update.
	       Changes in TOG templates
	       Corrected typo in ACM/IMS journals

Version 2.01   \acmPrice now produces a warning.

Version 2.00   ACM switches to electronic only version.
	       We do not print article tabs anymore.
	       New copyright wording.
	       Deleted \acmPrice.

Version 1.93   Added PACMSE

Version 1.92   Documentation update
	       Emergency change: changed order of hyperref and hyperxmp
	       due to changes in the undelying packages

Version 1.91   Minor changes in ACMCP format

Version 1.90a  Changes in the sample keywords and concepts

Version 1.90   Journal ISSN updated

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> figures/tables/page_migration.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{comment}
\begin{table*}[!t]
\caption{NUMA statistics with different page migration and placement strategies. }
\label{tab:pagemigration}
\vspace{-10pt}
\footnotesize
\resizebox{0.99\textwidth}{!}{

\begin{tabular}{|cc|rr|rr|rr|}
\hline
\multicolumn{2}{|l|}{}                                        & \multicolumn{2}{c|}{\textbf{AutoNUMA}}                                                                 & \multicolumn{2}{c|}{\textbf{Tiering-0.8}}                                                              & \multicolumn{2}{c|}{\textbf{TPP}}                                                                       \\ \cline{3-8} 
\multicolumn{2}{|l|}{\multirow{-2}{*}{}}                      & \multicolumn{1}{c|}{\textbf{hint\_faults}}             & \multicolumn{1}{c|}{\textbf{migrated\_pages}} & \multicolumn{1}{c|}{\textbf{hint\_faults}}             & \multicolumn{1}{c|}{\textbf{migrated\_pages}} & \multicolumn{1}{c|}{\textbf{hint\_faults}}              & \multicolumn{1}{c|}{\textbf{migrated\_pages}} \\ \hline
\multicolumn{1}{|c|}{}                           & First touch & \multicolumn{1}{r|}{336,469,816}                       & 3                                             & \multicolumn{1}{r|}{125,802,092}                       & 46                                            & \multicolumn{1}{r|}{4,654,013,085}                      & 5                                             \\ \cline{2-8} 
\multicolumn{1}{|c|}{\multirow{-2}{*}{\textbf{BTree}}}    & Interleave & \multicolumn{1}{r|}{6,092}     & 492                   & \multicolumn{1}{r|}{6,916}     & 51                    & \multicolumn{1}{r|}{5,092}      & 1                     \\ \hline
\multicolumn{1}{|c|}{}                           & First touch & \multicolumn{1}{r|}{31,793,182}                        & 117                                           & \multicolumn{1}{r|}{63,893,091}                        & 7,653,699             & \multicolumn{1}{r|}{5,894,907,183}                      & 6,929,247                                     \\ \cline{2-8} 
\multicolumn{1}{|c|}{\multirow{-2}{*}{\textbf{PageRank}}} & Interleave & \multicolumn{1}{r|}{28,398}    & 10,050                & \multicolumn{1}{r|}{613,906}   & 4,412                 & \multicolumn{1}{r|}{165,721}    & 15                    \\ \hline
\multicolumn{1}{|c|}{}                           & First touch & \multicolumn{1}{r|}{66,495,782}                        & 118,621                                       & \multicolumn{1}{r|}{398,259,304}                       & 6,134                                         & \multicolumn{1}{r|}{36,393,830,981}                     & 190                                           \\ \cline{2-8} 
\multicolumn{1}{|c|}{\multirow{-2}{*}{\textbf{Graph500}}} & Interleave & \multicolumn{1}{r|}{4,381,521} & 124                   & \multicolumn{1}{r|}{282,087}   & 6,114                 & \multicolumn{1}{r|}{74,432,220} & 1,569                 \\ \hline
\multicolumn{1}{|c|}{}                           & First touch & \multicolumn{1}{r|}{146,665,022}                       & 21,494                                        & \multicolumn{1}{r|}{220,094,592}                       & 3,264                                         & \multicolumn{1}{r|}{1,588,732,736}                      & 1,497,420                                     \\ \cline{2-8} 
\multicolumn{1}{|c|}{\multirow{-2}{*}{\textbf{Silo}}}     & Interleave & \multicolumn{1}{r|}{11,428}    & 10                    & \multicolumn{1}{r|}{5,581,434} & 14,512                & \multicolumn{1}{r|}{60,638}     & 0                     \\ \hline
\end{tabular}
}
\end{table*}

\end{comment}


\begin{table*}[!t] 
\centering
\caption{NUMA statistics with various page migration and static page placement solutions. \textcolor{red}{(remove this)}} 
\label{tab:pagemigration}
\vspace{-5pt}
\footnotesize
\resizebox{0.90\textwidth}{!}{
\begin{tabular}{
    |c|c|
    r|r|
    r|r|
    r|r|
}
\hline
\multicolumn{2}{|c|}{} & \multicolumn{2}{c|}{\textbf{AutoNUMA}} & \multicolumn{2}{c|}{\textbf{Tiering-0.8}} & \multicolumn{2}{c|}{\textbf{TPP}} \\ 
\cline{3-8} 
\multicolumn{2}{|c|}{\multirow{-2}{*}{}} & \textbf{hint\_faults} & \textbf{migrated\_pages} & \textbf{hint\_faults} & \textbf{migrated\_pages} & \textbf{hint\_faults} & \textbf{migrated\_pages} \\ 
\hline
\textbf{BTree} & \cellcolor{lightgray}First touch & \cellcolor{lightgray}336,469,816 & \cellcolor{lightgray}3 & \cellcolor{lightgray}125,802,092 & \cellcolor{lightgray}46 & \cellcolor{lightgray}4,654,013,085 & \cellcolor{lightgray}5 \\ 
\cline{2-8} 
 & Interleave & 6,092 & 492 & 6,916 & 51 & 5,092 & 1 \\ 
\hline
\textbf{PageRank} & \cellcolor{lightgray}First touch & \cellcolor{lightgray}31,793,182 & \cellcolor{lightgray}117 & \cellcolor{lightgray}63,893,091 & \cellcolor{lightgray}7,653,699 & \cellcolor{lightgray}5,894,907,183 & \cellcolor{lightgray}6,929,247 \\ 
\cline{2-8} 
 & Interleave & 28,398 & 10,050 & 613,906 & 4,412 & 165,721 & 15 \\ 
\hline
\textbf{Graph500} & \cellcolor{lightgray}First touch & \cellcolor{lightgray}66,495,782 & \cellcolor{lightgray}118,621 & \cellcolor{lightgray}398,259,304 & \cellcolor{lightgray}6,134 & \cellcolor{lightgray}36,393,830,981 & \cellcolor{lightgray}190 \\ 
\cline{2-8} 
 & Interleave & 4,381,521 & 124 & 282,087 & 6,114 & 74,432,220 & 1,569 \\ 
\hline
\textbf{Silo} & \cellcolor{lightgray}First touch & \cellcolor{lightgray}146,665,022 & \cellcolor{lightgray}21,494 & \cellcolor{lightgray}220,094,592 & \cellcolor{lightgray}3,264 & \cellcolor{lightgray}1,588,732,736 & \cellcolor{lightgray}1,497,420 \\ 
\cline{2-8} 
 & Interleave & 11,428 & 10 & 5,581,434 & 14,512 & 60,638 & 0 \\ 
\hline
\end{tabular}
}
\end{table*}

==> text/ann.tex <==
\section{Using CXL Memory on ANNS Applications}
\label{sec:ann_search}
This sections shows the impact of using CXL memory on Billion-scale Approximate Nearest Neighbor Search.

==> text/database.tex <==
\section{Using CXL Memory on Database Applications}
\label{sec:database}
This section shows the results of using CXL memory for commercial database applications, TPCC, TPCH, Redis, etc.

==> text/hpc.tex <==
\section{Using CXL Memory on HPC Applications}
\label{sec:hpc}
\subsection{System and Device}
\noindent \textbf{Systems.} We use a server to evaluate the latest commercial hardware supporting CXL memory. The server consists of 
two AMD EPYC 9354 CPU sockets. One socket is populated with eight 4800 MT/s DDR5 DRAM DIMMs (128 GB) across eight memory channels. The other socket is populated with only one 4800 MT/s DDR5 DRAM DIMM to emulate the bandwidth and capacity of CXL memory. The AMD EPYC 9354 CPU integrates four CPU chiplets, each with up to 8 cores and two DDR5 DRAM channels. We turn off the hyper-threading feature and set the CPU core clock frequency to 2.1 GHz for more predictable performance.

\noindent \textbf{CXL memory devices.} We take three CXL memory devices, each featuring different CXL IPs (DRAM-based(128GB) hard IP) and DRAM technologies (DDR5-4800). Since the CXL protocol itself does not prescribe the underlying memory technology, it can seamlessly and transparently accommodate not only DRAM but also persistent memory, flash, and other emerging memory technologies. Consequently, various CXL memory devices may exhibit different latency and bandwidth characteristics.


\textcolor{red}{(add the figure from the skype. Use Intel MCL. cachebench from Meta)}








\subsection{Runtime Comparison}
This sections characterizes the impact of using CXL memory on HPC workloads.

Finding1: Interleave0,1,2 policy have higher performance than interleave0,2 and interleave1,2. For two reasons: (1) The overall bandwidth becomes larger once interleaving over three NUMA nodes; (2) More memory are allocated on the DRAM, for interleave policy, memory are allocated in a round-robin way across all the involved NUMA nodes. That means for interleave0,1,2, memory is evenly allocated across three NUMA nodes (33.3\%), while for interleave0,1 and 1,2, 50\% of memory is allocated on DRAM and the rest 50\% of memory is allocated on CXL device. 

Finding1: Interleave0,1,2 policy have higher performance than interleave0,2 and interleave1,2. For two reasons: (1) The overall bandwidth becomes larger once interleaving over three NUMA nodes; (2) More memory are allocated on the DRAM, for interleave policy, memory are allocated in a round-robin way across all the involved NUMA nodes. That means for interleave0,1,2, memory is evenly allocated across three NUMA nodes (33.3\%), while for interleave0,1 and 1,2, 50\% of memory is allocated on DRAM and the rest 50\% of memory is allocated on CXL device.

\begin{figure*}[tb!]
	\centering
	\includegraphics[width=0.8\linewidth]{./figures/lu_cpu1.pdf}
	\caption{The runtime comparison when running LU workload class E, the memory consumption is 134GB.}
	\centering
	\label{fig:lu_cpu1} 
\end{figure*}
\begin{figure*}[tb!]
	\centering
	\includegraphics[width=0.8\linewidth]{./figures/cg_cpu1.pdf}
	\caption{The runtime comparison when running CG workload class E, the memory consumption is 134GB. There are three NUMA nodes, node0 and node1 are remote and local DRAM respectively, and node3 is the CXL device with 128GB memory capacity which is attached with socket1. We run the workload on socket1.}
	\centering
	\label{fig:cg_cpu1} 
\end{figure*}
\begin{figure*}[tb!]
	\centering
	\includegraphics[width=0.8\linewidth]{./figures/mg_cpu1.pdf}
	\caption{The runtime comparison when running MG workload class E, the memory consumption is 210GB.}
	\centering
	\label{fig:mg_cpu1} 
\end{figure*}
\begin{figure*}[tb!]
	\centering
	\includegraphics[width=0.8\linewidth]{./figures/sp_cpu1.pdf}
	\caption{The runtime comparison when running SP workload class E, the memory consumption is 174GB.}
	\centering
	\label{fig:sp_cpu1} 
\end{figure*}
\begin{figure*}[tb!]
	\centering
	\includegraphics[width=0.8\linewidth]{./figures/ft_cpu1.pdf}
	\caption{The runtime comparison when running FT workload class D, the memory consumption is 80GB.}
	\centering
	\label{fig:ft_cpu1} 
\end{figure*}
\begin{figure*}[tb!]
	\centering
	\includegraphics[width=0.8\linewidth]{./figures/xsbench_cpu1.pdf}
	\caption{The runtime comparison when running XSBench workload, the memory consumption is 116GB.}
	\centering
	\label{fig:xsbench_cpu1} 
\end{figure*}

==> text/intro_old.tex <==
\section{Introduction \textcolor{red}{(simplify)}}
\label{sec:intro}
Compute eXpress Link (CXL) is emerging as a promising memory interface technology. %%%built upon joint efforts between major hardware manufacturers (e.g., Intel~\cite{Intel_processor}, AMD~\cite{meta_amd, amd}, MICRON~\cite{Micron}, and SK Hynix~\cite{skhynix}) and hyperscalers (e.g., Meta~\cite{ 10.1145/3582016.3582063, meta_amd} and Microsoft~\cite{li2023pond}). 
Based on the standard PCIe serial interface, CXL can attach memory to the CPU and appears to a system as a CPU-less NUMA node. %This introduces flexibility in memory subsystem design and fine-grained control over memory bandwidth and capacity.
Compared with the traditional memory interface technology (such as DDR), CXL provides multiple benefits. \textit{First}, CXL provides a more scalable approach for increasing memory capacity and bandwidth without requiring additional DDR channels or causing a super-linear increase in energy consumption and signaling challenges, as seen with DDR~\cite{micro23_cxl}.
%CXL provides a more scalable method than DDR to increase memory capacity and bandwidth, because CXL does not increase the number of DDR channels or cause super-linear increase of energy consumption and signaling challenges as DDR~\cite{micro23_cxl}. %%\textit{Second}, the CXL memory provides a solution to avoid memory stranding~\cite{li2023pond},  because using the CXL memory as a pool, the stranded memory can be disaggregated from servers and provide memory capacity as demanded. 
\textit{Second}, with CXL, the memory technologies are decoupled from the memory interface technologies used by the CPU~\cite{wang2020characterizing, xiang2022characterizing, yang2020empirical}, which provides flexibility to reuse old memory and build the memory pool. \textit{Third},  CXL allows the CPU to communicate with the attached memory in a cache-coherent fashion using load and store instructions. This is aligned with traditional memory semantics, and hence provides conveniences of using existing programming models and system designs (e.g., NUMA-based tiered memory). \textit{Fourth}, data fetched from and written to the CXL memory can be cached in the cache hierarchy in the CPU, which allows the system to explore locality for higher performance. This contrasts with RDMA where data cannot be cached in the CPU. 




\begin{comment}
Compute eXpress Link (CXL) is emerging as a promising memory interface technology built upon joint efforts between major hardware manufacturers (e.g., Intel~\cite{Intel_processor}, AMD~\cite{meta_amd, amd}, MICRON~\cite{Micron}, and SK Hynix~\cite{skhynix}) and hyperscalers (e.g., Meta~\cite{ 10.1145/3582016.3582063, meta_amd} and Microsoft~\cite{li2023pond}). Based on the standard PCIe serial interface, CXL can attach memory to the CPU and appears to a system as a CPU-less NUMA node. This introduces flexibility in memory subsystem design and fine-grained control over memory bandwidth and capacity. As a result, CXL is poised to meet the ever-increasing requirements of memory bandwidth and memory capacity from data-intensive  applications (such as in-memory databases~\cite{lee2024database}, graph analysis~\cite{288782},  and scientific applications~\cite{yang2023cxlmemuring, wahlgren2022evaluating}). 

Compared with the traditional memory interface technology (such as DDR), CXL provides multiple benefits. First, CXL provides a more scalable method than DDR to increase memory capacity and bandwidth. The memory bandwidth and capacity is determined by the number of DIMMs per memory channel, the number of channels per CPU package, and the bit transfer rate~\cite{micro23_cxl}. DDR is not scalable because of super-linear increase of energy consumption and signaling challenges when increasing the number of DIMMs and data transfer rate. Also, given a CPU package, increasing the number of DDR channels for higher memory bandwidth leads to the addition of more pins, which is not scalable. For example, DDR5 requires 288 pins per channel~\cite{ddr4_5}. 
\end{comment}

\begin{comment}
Compared with the traditional memory interface technology (such as DDR), CXL provides multiple benefits. First, CXL provides a more scalable method than DDR to increase memory capacity and bandwidth. The memory bandwidth and capacity is determined by the number of DIMMs per memory channel, the number of channels per CPU package, and the bit transfer rate~\cite{micro23_cxl}. DDR is not scalable because of super-linear increase of energy consumption and signaling challenges when increasing the number of DIMMs and data transfer rate. Also, increasing the number of DDR channels for higher memory bandwidth leads to the addition of more pins in CPU package, which is not scalable.

Second, using CXL memory provides a solution to avoid memory stranding and hence save production cost in a data center. Memory stranding happens when all cores of a server are rented but there are unallocated memory capacity and cannot be rented. It has been reported that up to 25\% of DRAM is stranded in Microsoft Azure~\cite{li2023pond}. Using CXL memory as a pool, the stranded memory can be disaggregated from servers and provide memory capacity as demanded. 

Third, with CXL, the memory technologies are decoupled from the memory interface technologies used by the CPU. DDR4, DDR5, and persistent memory~\cite{wang2020characterizing, xiang2022characterizing, yang2020empirical} can all be connected to CPU by CXL. This provides unprecedented flexibility to reuse old memory and build the memory pool. 

Fourth, CXL allows the CPU to communicate with the attached memory in a cache-coherent fashion using load and store instructions. This is aligned with the traditional memory semantics, and hence provides conveniences of using existing programming models and system designs (e.g., NUMA-based tiered memory). Also, data fetched from and written to the CXL memory can be cached in each level of the cache hierarchy in the CPU, which allow the system to explore locality for higher performance. This contrasts with RDMA where data cannot be cached in the CPU. 
\end{comment}

%Compared with the traditional memory interface technology (such as DDR), CXL provides multiple benefits. \textit{First}, CXL provides a more scalable method than DDR to increase memory capacity and bandwidth, because CXL does not increase the number of DDR channels or cause super-linear increase of energy consumption and signaling challenges as DDR~\cite{micro23_cxl}. \textit{Second}, the CXL memory provides a solution to avoid memory stranding~\cite{li2023pond},  because using the CXL memory as a pool, the stranded memory can be disaggregated from servers and provide memory capacity as demanded. \textit{Third}, with CXL, the memory technologies are decoupled from the memory interface technologies used by the CPU~\cite{wang2020characterizing, xiang2022characterizing, yang2020empirical}, which provides unprecedented flexibility to reuse old memory and build the memory pool. \textit{Fourth},  CXL allows the CPU to communicate with the attached memory in a cache-coherent fashion using load and store instructions. This is aligned with traditional memory semantics, and hence provides conveniences of using existing programming models and system designs (e.g., NUMA-based tiered memory). \textit{Fifth}, data fetched from and written to the CXL memory can be cached in the cache hierarchy in the CPU, which \textcolor{sherry}{allows} the system to explore locality for higher performance. This contrasts with RDMA where data cannot be cached in the CPU. 



However, CXL memory introduces longer memory access latency.  This longer latency comes from PCIe, %(e.g., \~ 40 ns in PCIe 4.0), 
CXL memory controller, and CXL home agent (HA) on the CPU.  Figure~\ref{fig:latency_breakdown} compares local NUMA, traditional remote NUMA, and CXL-based memory expansion in terms of memory latency. %%%It has been reported that the CXL adds about 70-150 $ns$ of extra latency over normal DRAM access~\cite{10.1145/3582016.3582063}.

\begin{figure}[tb!]
	\centering
	\includegraphics[width=0.9\linewidth]{./figures/latency_breakdown.pdf}
	\caption{Breakdown of CXL memory access latency.}
	\centering
	\label{fig:latency_breakdown}
        \vspace{-20pt}
\end{figure}
%%The server B has the almost same organization as server A, the only difference is that the CXL memory on server B is attached with CPU0 not CPU1, while the server C has the same organization as server A}.


Given the CXL performance, we face a series of questions: what are the use cases for the CXL memory? What are the impacts of real CXL memory on application performance? At the application level, how to use the CXL memory in combination with fast memory components (e.g., using uniform page-level interleaving vs. data object-level interleaving vs. memory binding)? %How do the existing page management systems perform in the real CXL hardware?  
This paper aims to discuss those questions, characterize the performance of the CXL memory, and explore various paths to use the CXL memory. We study three genuine CXL memory expansion cards from different vendors. %%%%and have the following insights. 
%three genuine CXL-ready systems (\textcolor{dong}{including three CXL memory expansion cards from different memory vendors}), and have the following insights. %%%using ASIC-based hard CXL IPs.


\textbf{The CXL memory is a unique ``NUMA node''.}  The CXL memory appears as a CPU-less NUMA node. In the three systems we evaluate, the CXL memory appears as a two-hop-away NUMA node in terms of access latency. Depending on the memory vendors, the peak bandwidth of the CXL memory varies a lot, ranging from 9.8\% to 80.3\% of the peak bandwidth of local DRAM. %In addition, as we scale the number of threads to access the CXL memory, its memory bandwidth is easily saturated because of \textcolor{check}{single DRAM channel} (the saturation point is reached when the number of threads is only 4), while local DRAM (or LDRAM for short) and remote DRAM-based NUMA node (or RDRAM for short) have much better scalability. 
Moreover, as we increase the number of threads accessing the CXL memory, its bandwidth is quickly saturated due to \textcolor{ren}{the limited data transfer rate in CXL attached memory instead of PCIe bus — with saturation occurring when the number of threads reaches just four. }
In contrast, local DRAM (LDRAM) and remote DRAM-based NUMA nodes (RDRAM) exhibit much better scalability. 
This scaling difference between the CXL memory and DRAM highlights the importance of appropriately distributing memory accesses between them for high performance. Also, when the system is under heavy load, %we notice that LDRAM and RDRAM can show the similar latency as the CXL memory because of the contention on the memory controller (MC) or data path, which shows the potential of using CXL as LDRAM or RDRAM for latency-sensitive applications when the system is under heavy load. 
\textcolor{check}{we observe that the latencies of LDRAM and RDRAM are similar to that of the CXL memory because of the contention on the memory controller (MC) or data path, which shows the potential of using CXL as LDRAM or RDRAM for latency-sensitive applications under heavy load.}


\textbf{Using the CXL memory for large language models (LLM) faces challenges.} We study the cases that use the CPU memory as an extension to the GPU memory to enable LLM training (using ZeRO-Offload~\cite{atc21:zerooffload}) and inference (using FlexGen~\cite{flexgen}) such that we can use less GPUs for LLM without the constraint of GPU memory capacity. This method has to frequently copy tensors between the GPU and CPU, and offloads certain computations from the CPU to the GPU to maximize GPU memory saving or reduce I/O offload. This method (named \textit{tensor offloading} in the rest of the paper) has been commonly studied and deployed in industry. 

We find that using tensor offloading based upon the CXL memory brings limited performance improvement. This is because the tensor copy between the CXL memory and GPU memory goes through a longer data path than memory accesses directly from CPU. Using CXL 1.1 on our platform, this data path is bottlenecked by the PCIe interconnect between CPU and GPU. As a result, adding CXL cannot show the bandwidth benefits for tensor offloading. In contrast, the computation offloaded to the CPU (i.e., the optimizer for LLM training and the attention computation for LLM inference), which tends to be bandwidth sensitive, can benefit from the extra bandwidth of CXL.
%suffers from the performance loss when using CXL. As a result, using the CXL memory for tensor offloading cannot show obvious performance improvement. 
In addition, the CXL memory increases memory capacity and allows us to use larger batch sizes for LLM inference, leading to throughput gains. \textcolor{check}{Our study is unprecedented, because of its practicality of using real CXL for GPU-based LLM, different from CPU-based study~\cite{eurosys24_cxl}.}
%%%Compared to using NVMe, using the CXL memory shows performance benefits, because of the large capacity of the CXL memory, we are able to use larger batch size for LLM inference, which leads to throughput gains.  %%%\textcolor{red}{(pending to add a couple of more sentences.)}


%\textbf{HPC applications can benefit a lot from the CXL memory for high performance while saving fast memory.} 
\textbf{\textcolor{check}{CXL can be used to save fast memory without causing performance loss, and using application semantics to guide page interleaving for CXL can maximize CXL benefits.}} 
%Previous work~\cite{micro23_cxl} reveals that complex applications (e.g., social network microservices) exhibiting $ms$-scale latency experience a marginal increase in tail latency even when most of pages are allocated to CXL memory. 
Our work goes beyond the existing work~\cite{micro23_cxl, eurosys24_cxl} that focuses on applications exhibiting $ms$-scale latency (e.g., social network microservices) or commercial workloads to study the potential of the CXL memory. We study a spectrum of HPC workloads, covering the most common and representative ``HPC dwarfs''~\cite{Asanovic+:TR06}. We reveal that some HPC applications \textcolor{check}{(such as CG and BT~\cite{NPB})} can tolerate the low bandwidth and high latency of the CXL memory under certain scales (the performance loss is less than 3.2\%, compared with LDRAM), because of their compute-intensive nature. %%%%%\textcolor{check}{Even for a latency-sensitive application, using CXL memory can bring high performance, transforming high bandwidth to the latency reduction.}
%%%%%We also observe that the bandwidth-sensitive and latency-sensitive applications respond differently to the CXL performance. %%\textcolor{red}{As we scale the number of threads, the bandwidth-sensitive application narrows down the performance difference between using CXL and not using CXL, because of the bandwidth benefit offered by CXL}, while the latency-sensitive application increases the difference. 

In addition, the page interleaving policy, embraced by the industry (e.g., Micron and AMD~\cite{micron_hetero_interleaving}, Astera Labs~\cite{asteralabs_hetero_interleaving}, and Samsung~\cite{samsung_hetero_interleaving}) as an application-transparent technique to integrate CXL with the existing memory components, provides opportunities to save LDRAM for HPC applications. When interleaving CXL and RDRAM,  we see minor performance difference from interleaving CXL and LDRAM for some applications. This is because the CXL memory dominates the memory performance, and the performance of other memory components has minor impact on the overall performance. 

To maximize the interleaving performance, we introduce a novel data object-level interleaving %\textcolor{sherry}{(or object-level interleaving for short)} 
policy.  
%\textcolor{sherry}{Different from the Linux uniform page-level interleaving (or uniform interleaving for short)  policy~\cite{micro23_cxl}}, 
Different from Linux uniform page-level interleaving~\cite{micro23_cxl}, this policy decides whether memory pages allocated to a data object should be interleaved between CXL and DRAM or allocated to LDRAM first (``LDRAM preferred''). This policy maximizes memory bandwidth (or minimizes latency) for data objects whose accesses favor high bandwidth (or low latency). %and minimizes the latency for data objects whose accesses favor low latency. 
This policy reduces LDRAM usage by \textcolor{check}{$32\%$} and outperforms the uniform interleaving policy (Linux default) by $65\%$ on average.




\textbf{Memory tiering solutions need to be improved.} Treating the CXL memory as a memory tier, existing work~\cite{autonuma, tiering0.8, eurosys24:mtm, 10.1145/3582016.3582063, Raybuck2021HeMemST, 10.1145/3600006.3613167} migrates pages between the CXL memory and fast memories based on page access frequency or recency (i.e., hotness). Those solutions are seldom studied with the real CXL memory, and \textit{how they interplay with the existing system (e.g., page interleaving) is largely unknown.} 

We find that the dynamic page migration in the memory tiering solutions are not integrated well with the static page interleaving,  because of invalidness of NUMA hint faults. Depending on the temporal and spatial distribution of hot pages, the dynamic page migration can degrade application performance compared to no migration.
%Depending on the hot page distribution in time and address space, the dynamic page migration can lose application performance, compared with no migration. 
We also observe that the old-fashioned NUMA first touch and Tiering-0.8~\cite{tiering0.8} (the most recent Linux Patch for AutoNUMA to support memory tiering) is very effective, outperforming a set of page migration and interleaving solutions.








%%%\textbf{Existing page management systems for tiered memory face challenges on the CXL memory.} 


==> text/model_inference.tex <==
\section{Using CXL Memory on LLM Inference}
\label{sec:llm_inference}
This sections shows the impact of using CXL memory on Large Language Model inference performance.
